Interactive Proofs of Proximity for Model Evaluation

We study interactive proofs of proximity (IPPs) for model evaluation, where a resource-limited verifier interacts with an untrusted prover, typically the model owner, to certify statistical properties of a model under an unknown input distribution. Our formulation separates sampling the input distribution from querying the model and evaluating its output; distinguishes real audit data (black-box sampling) from generated data (chosen-randomness, or gray-box, access to the sampler); and allows the prover and verifier to use different evaluators. We focus on doubly-sublinear IPPs, where both the verifier and honest prover use sublinear resources, and on (weighted) Hamming weight properties. For ordinary Hamming weight, we give a tolerant doubly-sublinear IPP. For completeness and soundness radii $\varepsilon_c<\varepsilon_f$ and gap $g=\varepsilon_f-\varepsilon_c$, a logarithmic-round instantiation uses $\widetilde{O}(1/g)$ verifier queries and $O(1/g^2)$ honest-prover queries, improving the cubic dependence of Amir, Goldreich, and Rothblum (ITCS 2025). We prove matching query lower bounds up to polylogarithmic factors. For distribution-weighted Hamming weight, black-box sampling requires $\Theta(1/g^2)$ verifier samples but only $\widetilde{O}(1/g)$ evaluations; the quadratic sample complexity is necessary in the interior regime. With chosen-randomness access, the problem reduces to ordinary Hamming weight, yielding $\widetilde{O}(1/g)$ calls and evaluations. If the parties' evaluators disagree arbitrarily on a $\rho$-fraction of the distribution and by at most $\gamma$ elsewhere, our protocols remain doubly sublinear whenever $g>2\kappa$, where $\kappa=\rho+(1-\rho)\gamma$. Applications include auditing accuracy, group fairness, calibration, harmlessness, usefulness, and average-case robustness.

==> packages.tex <==
\RequirePackage{fix-cm}
\usepackage[margin=1.1in]{geometry}
\usepackage{mathtools,amssymb,amsthm}
%%%%%%%% Font packages %%%%%%%%%%%%%%%%
\ifnum\bland=0
\usepackage[T1]{fontenc}
\usepackage{erewhon}
\usepackage[utopia,vvarbb]{newtxmath}
\usepackage{microtype}
\usepackage{mleftright}
\mleftright
\frenchspacing
\raggedbottom
\else
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{booktabs}
\usepackage{verbatim}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xcolor}
\usepackage[colorlinks=true,linkcolor=blue!60!black,citecolor=blue!60!black,urlcolor=blue!60!black]{hyperref}
\usepackage{tikz}
\usepackage{todonotes}
\usepackage{natbib}
\usepackage{placeins}
\usepackage{xparse}
\usepackage[most]{tcolorbox}
\usetikzlibrary{arrows.meta,calc,positioning}
\usepackage{authblk}
\usepackage{titlesec}
